CoVR-2: Automatic Data Construction for Composed Video Retrieval

Composed Image Retrieval (CoIR) has recently gained popularity as a task that considers both text and image queries together, to search for relevant images in a database. Most CoIR approaches require manually annotated datasets, comprising image-text-image triplets, where the text describes a modification from the query image to the target image. However, manual curation of CoIR triplets is expensive and prevents scalability. In this work, we instead propose a scalable automatic dataset creation methodology that generates triplets given video-caption pairs, while also expanding the scope of the task to include composed video retrieval (CoVR). To this end, we mine paired videos with a similar caption from a large database, and leverage a large language model to generate the corresponding modification text. Applying this methodology to the extensive WebVid2M collection, we automatically construct our WebVid-CoVR dataset, resulting in 1.6 million triplets. Moreover, we introduce a new benchmark for CoVR with a manually annotated evaluation set, along with baseline results. We further validate that our methodology is equally applicable to image-caption pairs, by generating 3.3 million CoIR training triplets using the Conceptual Captions dataset. Our model builds on BLIP-2 pretraining, adapting it to composed video (or image) retrieval, and incorporates an additional caption retrieval loss to exploit extra supervision beyond the triplet. We provide extensive ablations to analyze the design choices on our new CoVR benchmark. Our experiments also demonstrate that training a CoVR model on our datasets effectively transfers to CoIR, leading to improved state-of-the-art performance in the zero-shot setup on the CIRR, FashionIQ, and CIRCO benchmarks. Our code, datasets, and models are publicly available at https://imagine.enpc.fr/~ventural/covr/.

==> 5c_bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1.0in,clip,keepaspectratio]{figures/bios/lucas.png}}]{Lucas Ventura}
    received the BSc and MSc degrees in Telecommunications Engineering from Universitat Polit\`ecnica de Catalunya (UPC), Barcelona in 2016 and 2018, respectively.
    He is currently pursuing a PhD in the IMAGINE computer vision team at \'{E}cole des Ponts ParisTech (ENPC) and the WILLOW team at Inria Paris, under the co-supervision of G\"{u}l Varol and Cordelia Schmid. His research interests include deep learning and computer vision, with a particular focus on unsupervised learning, video representation learning, and text-video integration.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1.0in,clip,keepaspectratio]{figures/bios/antoine.jpg}}]{Antoine Yang}
    is a Research Scientist at Google DeepMind in London, working on the multi-modal capabilities of Gemini. In 2023, he completed his PhD in the WILLOW team of Inria Paris and \'{E}cole Normale Sup\'{e}rieure, advised by Antoine Miech, Josef Sivic, Ivan Laptev and Cordelia Schmid. His thesis, supported by a Google PhD Fellowship, focused on learning visual language models for video understanding. In 2020, he received an engineering degree from \'{E}cole Polytechnique and a MSc degree in Mathematics, Vision and Learning from ENS Paris-Saclay. 
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1.0in,clip,keepaspectratio]{figures/bios/cordelia.jpg}}]{Cordelia Schmid}
    holds a M.S. degree in Computer Science from the University of Karlsruhe and a Doctorate, also in Computer Science, from the Institut National Polytechnique de Grenoble (INPG). Her doctoral thesis on "Local Greyvalue Invariants for Image Matching and Retrieval" received the best thesis award from INPG in 1996. She received the Habilitation degree in 2001 for her thesis entitled "From Image Matching to Learning Visual Models". Dr. Schmid was a post-doctoral research assistant in the Robotics Research Group of Oxford University in 1996--1997. Since 1997 she has held a permanent research position at Inria, where she is a research director.
    
    Dr. Schmid is a member of the German National Academy of Sciences, Leopoldina and a fellow of IEEE and the ELLIS society. She was awarded the Longuet-Higgins prize in 2006, 2014 and 2016, the Koenderink prize in 2018 and the Helmholtz prize in 2023, all for fundamental contributions in computer vision that have withstood the test of time. She received an ERC advanced grant in 2013, the Humboldt research award in 2015, the Inria \& French Academy of Science Grand Prix in 2016, the Royal Society Milner award in 2020 and the PAMI distinguished researcher award in 2021. In 2023 she received the K\"{o}rber European Science Prize and in 2024 the European Inventor Award in the research category. Dr. Schmid has been an Associate Editor for IEEE PAMI (2001--2005) and for IJCV (2004--2012), an editor-in-chief for IJCV (2013--2018), a program chair of IEEE CVPR 2005 and ECCV 2012 as well as a general chair of IEEE CVPR 2015, ECCV 2020 and ICCV 2023. Starting 2018 she holds a joint appointment with Google research.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1.0in,clip,keepaspectratio]{figures/bios/gul.jpg}}]{G\"ul Varol}
    is a permanent researcher in the IMAGINE group at \'{E}cole des Ponts ParisTech. Previously, she was a postdoctoral researcher at the University of Oxford (VGG). She obtained her PhD from the WILLOW team of Inria Paris and \'{E}cole Normale Sup\'{e}rieure (ENS). Her thesis received the PhD awards from ELLIS and AFRIF. During her PhD, she spent time at MPI, Adobe, and Google. Prior to that, she received her BS and MS degrees from Bogazici University. She regularly serves as an Area Chair at major computer vision conferences and is serving as a Program Chair at ECCV'24. She is an associate editor for IJCV and was in the award committee for ICCV'23. She has co-organized a number of workshops at CVPR, ICCV, ECCV, and NeurIPS. Her research interests cover vision and language applications, including video representation learning, human motion synthesis, and sign languages.
\end{IEEEbiography}

